Empirical analysis of metaheuristic search techniques for the parameterized dynamic slope scaling procedure

The dynamic slope scaling procedure is an approximation method successfully which solves the fixed charge network flow (FCNF) problem by iteratively linearizing the fixed cost. The parameterized dynamic slope scaling procedure adds an additional $\psi$ parameter to the procedure which can significantly improve the solution quality. Finding the optimal value of $\psi$ for a given problem is non-trivial. This paper employs multiple metaheuristic techniques, including simulated annealing, tabu search, and particle swarm optimization, to guide the search for good parameter values. In rigorous testing, we examine the search results, compare the improvement efficiencies among the techniques, and evaluate the final solution quality of the FCNF problem. The experiments show that the solution improvement is robust with respect to these metaheuristics and the complexity of FCNF problem.

==> PSO_line_search.tex <==
\begin{tikzpicture}[scale=1]

%begin graph on left ---------
\footnotesize
% line
\draw[thick] (-6.5,0) -- (6.5,0); % node[anchor=north] {$M_{ij}$};

		
% ticks and labels
\draw[-] (-6,-0.1) -- (-6,0.1);
\draw	(-6,-0.1) node[anchor=north] {$-h_3$};

\draw[-] (-3,-0.1) -- (-3,0.1) ; %node[anchor=east] {$z_{ij}$};
\draw	(-3,-0.1) node[anchor=north] {$-h_2$};

\draw[-] (-1.5,-0.1) -- (-1.5,0.1) ; %node[anchor=east] {$z_{ij}$};
\draw	(-1.5,-0.1) node[anchor=north] {$-h_1$};

\draw[-] (-0.25,-0.1) -- (-0.25,0.1) ; %node[anchor=east] {$z_{ij}$};
\draw	(-.3,-0.1) node[anchor=north] {$-h_0$};

\draw[-] (6,-0.1) -- (6,0.1) ; %node[anchor=east] {$z_{ij}$};
\draw	(6,-0.1) node[anchor=north] {$h_3$};

\draw[-] (3,-0.1) -- (3,0.1) ; %node[anchor=east] {$z_{ij}$};
\draw	(3,-0.1) node[anchor=north] {$h_2$};

\draw[-] (1.5,-0.1) -- (1.5,0.1) ; %node[anchor=east] {$z_{ij}$};
\draw	(1.5,-0.1) node[anchor=north] {$h_1$};

\draw[-] (0.25,-0.1) -- (0.25,0.1) ; %node[anchor=east] {$z_{ij}$};
\draw	(.3,-0.1) node[anchor=north] {$h_0$};

%add neighbor points
\draw [fill] (0,0) circle [radius=0.075];
\draw (0,0.1) node[anchor=south] {$\psi_i$};

\draw [fill] (1,0) circle [radius=0.075];
\draw (1,0.1) node[anchor=south] {$\psi_{i,1}$};

\draw [fill] (-1.85,0) circle [radius=0.075];
\draw (-1.85,0.1) node[anchor=south] {$\psi_{i,2}$};

\draw [fill] (5.5,0) circle [radius=0.075];
\draw (5.5,0.1) node[anchor=south] {$\psi_{i,3}$};

\end{tikzpicture}



